Microstructure-Empowered Stock Factor Extraction and Utilization

High-frequency quantitative investment is a crucial aspect of stock investment. Notably, order flow data plays a critical role as it provides the most detailed level of information among high-frequency trading data, including comprehensive data from the order book and transaction records at the tick level. The order flow data is extremely valuable for market analysis as it equips traders with essential insights for making informed decisions. However, extracting and effectively utilizing order flow data present challenges due to the large volume of data involved and the limitations of traditional factor mining techniques, which are primarily designed for coarser-level stock data. To address these challenges, we propose a novel framework that aims to effectively extract essential factors from order flow data for diverse downstream tasks across different granularities and scenarios. Our method consists of a Context Encoder and an Factor Extractor. The Context Encoder learns an embedding for the current order flow data segment's context by considering both the expected and actual market state. In addition, the Factor Extractor uses unsupervised learning methods to select such important signals that are most distinct from the majority within the given context. The extracted factors are then utilized for downstream tasks. In empirical studies, our proposed framework efficiently handles an entire year of stock order flow data across diverse scenarios, offering a broader range of applications compared to existing tick-level approaches that are limited to only a few days of stock data. We demonstrate that our method extracts superior factors from order flow data, enabling significant improvement for stock trend prediction and order execution tasks at the second and minute level.

==> Change_Zizhong.tex <==
1. 把intro删掉的引用加在了第二句话后面
2. 把所有 timestamp segment的表述换成了 order segment，和Figure3一致
3. 改了page2左栏的一句话：Then, we employ separate generators for bid and ask orders, while incorporating shared information to generate future orders. 
4. Contribution（3）表述调整了下


==> abs_Chang.tex <==
\begin{abstract}

High-frequency quantitative investment is a crucial aspect of stock investment.
Notably, \textit{order flow data} plays a critical role as it provides the most detailed level of information among high-frequency trading data, including comprehensive data from the \textit{order book} and \textit{transaction} records at the tick level. 
The order flow data is extremely valuable for market analysis as it equips traders with essential insights for making informed decisions.
However, extracting and effectively utilizing order flow data present challenges due to the large volume of data involved and the limitations of traditional factor mining techniques, which are primarily designed for coarser-level stock data.
To address these challenges, we propose a novel framework that aims to effectively extract essential factors from order flow data 
for diverse downstream tasks across different granularities and scenarios.
Our method consists of a Context Encoder and an Factor Extractor. The Context Encoder learns an embedding for the current order flow data segment's context by considering both the expected and actual market state. 
In addition, the Factor Extractor uses unsupervised learning methods to select such important signals that are most distinct from the majority within the given context. 
The extracted factors are then utilized for downstream tasks. 
In empirical studies, our proposed framework efficiently handles an entire year of stock order flow data across diverse scenarios, offering a broader range of applications compared to existing tick-level approaches that are limited to only a few days of stock data.
We demonstrate that our method extracts superior factors from order flow data, enabling significant improvement for stock trend prediction and order execution tasks at the second and minute level.
%Our approach significantly outperforms other microstructure-based factor mining methods.
\end{abstract}

==> tmp.tex <==
In this section, we will provide a detailed description of our approach for extracting microstructure factors from large-scale order flow data and demonstrate their utilization in downstream tasks. 
To handle the substantial volume of order flow-level data, we divide it into smaller segments and extract features from segments. 
In addition, we propose to consider the context of each segment during feature extraction.
In Section 3.1, we introduce how to encode historical information as market condition information by Context Encoder.
Section 3.2 presents our Informative Factor Extractor module. 
To extract general factors applicable to diverse downstream tasks and temporal granularities, we adopt unsupervised methods that do not rely on task-specific label information during feature extraction. 
Moreover, to apply the extracted information from the segments to tasks at coarser time granularity, we employ a selection mechanism that identifies the most influential subset of segments based on their deviations from the majority within the given context. 
We will now delve into a more comprehensive explanation of our proposed model.





